Discovering Biases in Information Retrieval Models Using Relevance Thesaurus as Global Explanation

Most efforts in interpreting neural relevance models have focused on local explanations, which explain the relevance of a document to a query but are not useful in predicting the model's behavior on unseen query-document pairs. We propose a novel method to globally explain neural relevance models by constructing a "relevance thesaurus" containing semantically relevant query and document term pairs. This thesaurus is used to augment lexical matching models such as BM25 to approximate the neural model's predictions. Our method involves training a neural relevance model to score the relevance of partial query and document segments, which is then used to identify relevant terms across the vocabulary space. We evaluate the obtained thesaurus explanation based on ranking effectiveness and fidelity to the target neural ranking model. Notably, our thesaurus reveals the existence of brand name bias in ranking models, demonstrating one advantage of our explanation method.

==> 2_related_bk.tex <==
\section{Related works}
Our work is closely related to vocabulary mismatch problem, which refer to the situation where there's a discrepancy between the words used in a query and the words used in the relevant documents~\cite{croft2010search}.

 First we describe the works on traditional information retrieval methods that are before the use of large language models. Then we will move to large language model based approaches and describe how our work differs from them. Lastly, we will describe our works implications to broader text modeling field.

\subsection{Traditional Information Retrieval}
Vocabulary mismatch problem was big problem in traditional information retrieval methods.
One of the widely used techniques for vocabulary mismatch is query expansion, which expands the original query with additional terms.
Query expansion is often based on word or term co-occurrences~\cite{jing1994association, xu2000improving}, and pseudo-relevance feedback (PRF) is one of the most popular techniques. 

\citet{berger1999information} adopted an idea of the statistical machine translation model~\cite{brown1990statistical} into the language model framework~\cite{ponte1998language} to handle vocabulary mismatch. A query was viewed as a translation of the document, and relevance probability is estimated based on probability that the query is translated from the given document. The translation probability of a query term translated into a specific document term is estimated based on the co-occurrence statistics in the collection.

The main difference of our work to previous traditional query expansion techniques is that we aim at utilizing the large language model fine-tuning instead of incorporating term co-occurrence or PRF. 
 
\subsection{Neural Information Retrieval}

Fine-tuning pre-trained language models, such as BERT \cite{devlin-etal-2019-bert}, has proven to be effective for information retrieval~\cite{macavaney2019cedr}. 
There are two popular categories methods which are purely based on distributed representations. The first is the cross-encoder architecture~\cite{dai2019deeper}, which encodes both the query and document at the same time in a single Transformer network, with allowing attention between all the tokens. The second is the bi-encoder architecture~\cite{formal2021splade}, where each of query and document are encoded separately into vectors and the dot product between the query vector and document vector is used to compute the score for the pair. These methods do not allow tracking which tokens of the query and which tokens of the document are relevant.
However, few studies have proposed a method to explicitly identify the relevance relation between query and document terms in order to construct a relevance scoring or retrieval function. 

There are methods that takes hybrid approaches, which use both the LLMs and term-level matching mechanisms.

There are neural query expansion or document expansion methods, which uses LLMs to add terms to the bag of word representations of a query or document, and retrieval is done with traditional methods. 
\citet{naseri2021ceqe} used LLM to generate expansion query terms for the query and used expanded query representation to perform traditional retrieval.
\citet{nogueira2019doc2query} used similar approach but instead encode the document to get expanded document terms. 
These method still does not explain which of the original query term and which original document terms are related, because retrieval and scoring is done by expanded query (document) terms.
 Moreover, these expansions are only applicable for individual query and document, cannot be used to describe global matching behavior for the retrieval system. 

 Multi-vector retrieval model such as ColBERRT~\cite{khattab2020colbert} and COIL~\cite{gao2021coil} can be considered as a special case of bi-encoder. They construct vector representations for each token in both the query and the document. They then utilize the similarity between the query-token vectors and the document-token vectors to compute the relevance score. Although they provide token-level interaction scores, these cannot entirely be attributed to their corresponding tokens. This is because the vector representation is already the result of contextualization and could be affected by other tokens in the sequence. Thus, the same term may have different representations across various documents, and we cannot acquire relevant terms from these models.

Splade~\cite{formal2021splade} is a sparse retrieval method, which encodes a query or document into a sparse vector.
Each vector's dimension is aligned with the subword vocabulary of BERT. 
However, this encoding process still exhibits unpredictability; the impact of specific tokens on the encoded vector's dimensions is not straightforward.
For example, the inclusion of the token ``is'' in the input does not guarantee a high weight for ``is'' in the corresponding dimensions of the output vector.

All of methods described above incur additional computational and/or storage overhead compared to the traditional retrieval. Bi-encoder models including Splade, require encoding all the corpus with the expensive neural network and storing the vector representations. Also, the storage required for the encoded vectors can be much larger than the storage for original documents. Efficient neural encoding of query or document requires special hardware acceleration, which is not be available in traditional servers. 

In contrast, the output model of our work is a table that indicates relation between the terms that are compatible to the traditional indexing architectures, and thus can be seamlessly augmented into existing infrastructures. Moreover all the computational overheads are during the training phase and does not incur significant overheads during the indexing or inference time.


\citet{boytsov2021exploring} extended the idea of translation language model\cite{berger1999information} by using BERT~\cite{devlin-etal-2019-bert} to estimate translation probability. The translation probability is estimated using a multilayer perceptron (MLP) model, where input is the concatenation of the (sub)word embeddings of the query term and document term. The MLP is trained end-to-end using the pairwise loss on MSMARCO training dataset. To make the model robust, this subword-level translation language model was combined with word-level (space-tokenized) BM25 scores to make it more robust. This work does not provide solution for how to model translation probability for the terms that are composed of multiple subwords in BERT's tokenization. Moreover, this model only uses the word-embeddings components of BERT and does not exploit full capacity of the Transformer network.


% \subsection{Global model explanations}

% Extracting decision trees from neural networks as global explanations is common~\cite{boz2002extracting}. The fidelity is evaluated as portion of data point that have the same classification output as the targeted neural network. 



==> Backup/1_intro_YK_version.tex <==
\section{Introduction}
Transformer-based information retrieval models~\cite{dai2019deeper, macavaney2019cedr} that are trained on large dataset like MS MARCO~\cite{msmarco} are very effective in predicting relevance between a query and document. We can expect that these models  capture \textit{semantic matches} such as a query term ``car'' to be matched to a document term ``vehicle''. However, it is challenging for researchers to predict when a model might fail, such as when it matches a query term to non-relevant document terms. 

Another potential risk associated with ranking models is unintended bias toward certain entities or groups. While it is appropriate for a model to associate the query term ``car'' with various car brand names (e.g., Ford), it is not desirable for the model to exhibit a strong preference for a particular brand, leading to the model favoring one brand over another when all other factors are identical.
 \input{table/ex_table}

Explanation methods for a machine learning model can be categorized into local or global~\cite{guidotti2018survey}, 
where local explanations target individual model predictions, such as a given query-document pair~\cite{kim2022alignment} or a ranked list for a query~\cite{LIRME, llordes2023explain}. Global explanations on the other hand aim to provide patterns underlying a model's behavior which are not restricted to specific instances.  

For the safe deployment of information retrieval (IR) models in real-world scenarios, 
analyzing global explanations for retrieval models is crucial 
because it can reveal insights that cannot necessarily be obtained from local explanations alone. 

This work aims at constructing global explanations for ranking models that can 
 assist in understanding neural ranking models and help identify potential risks. Specifically, we seek to identify relevant pairs of query terms and document terms that can effectively explain  the behavior of neural ranking models. We refer to this format of explanation as a \textit{relevance thesaurus}, as illustrated in Table~\ref{ex:table}. That table indicates that if a query contains the term ``injury'' then it is likely to correspond to document terms ``injure,'' or ``wound,'' with the first most likely, allowing a retrieval's results to be explained directly using the term pairs.

We focus on identifying the relevant term pairs that are context independent (e.g., synonyms) because they are more widely applicable and more feasible to evaluate than the context-sensitive term pair which are only relevant in specific contexts. This requirement makes many existing token-level IR models or local explanation methods not applicable to our goal, as they do not have mechanisms to isolate the effects of the context. Existing ranking models themselves are not designed to directly infer which are context-independently relevant terms pairs. Attention scores or inner products of token-representations are already the result of incorporating the contexts. 

Constructing a relevance thesaurus poses a challenge due to the large number of potential term pairs. Many local and global explanation methods explicitly build a candidate set of features from data and determine the appropriateness of each feature by assigning and adjusting scores using various optimization methods. However, this strategy becomes infeasible when the number of features increases, as in our case where the term pairs can scale to billions. To overcome this challenge, we propose a novel approach that implicitly optimizes the per-feature scores using an intermediate neural model called the Partial Relevance Model (PaRM). PaRM is designed to predict a score for a term pair, which is then used to predict the score for the query-document pair to which the term pair belongs. By training PaRM to mimic the behavior of the target cross-encoder model, we ensure that the generated relevance thesaurus faithfully explains the target model's behavior.

Rather than assessing the accuracy of each row in the relevance thesaurus, it is extrinsically evaluated by adding it into the traditional IR framework with BM25 scoring, thus incorporating a type of semantic matching. The resulting retrieval method is evaluated based on ranking effectiveness and the fidelity to the targeted neural ranking models.
The results on multiple datasets show the effectiveness of the acquired relevance thesaurus.

Our manual inspection of the relevance thesaurus, reveals three unexpected findings about the behavior of neural ranking models trained on MS MARCO: (1) the \textit{postfix-a} finding, which reveals that models treat the character ``a'' appended to a term as equivalent to a quotation mark due to encoding errors; (2) the \textit{car-brand bias}, which suggests that models exhibit biases towards certain car brands; (3) the \textit{temporal bias}, which indicates that models consider distant future or past years to be more strongly associated with the query term ``when'' compared to the current year. Experiments using multiple state-of-the-art neural information retrieval models demonstrate that these behaviors are not limited to the cross encoder but are replicated in multiple IR models, highlighting the value of our explanation method.

==> Draft/1_intro.tex <==
\section{Introduction}

\subsection{Motivation }

Explaining decisions of a machine learning model can be local or global~\cite{guidotti2018survey}. 
Local explainability provides explanations for individual model predictions. In information retrieval, it is for a given query-document pair~\cite{kim2022alignment} or a ranked list for a query~\cite{LIRME, llordes2023explain}. Global explanations on the other hand aim to provide patterns underlying a model's behavior which is not restricted to specific instances. 

A global explanation of retrieval models is crucial for the safe deployment of retrieval models in real-world scenarios because it can reveal insights that cannot be obtained from local explanations. 

\input{table/honda_ex}
As an example, for the query-document pair shown in Table~\ref{tab:qd_honda_actuator}, a feature-based local explanation could attributes a significant weight to the term ``Honda'' within the passage.
This behavior seems highly reasonable for the ranker. However, through our proposed global explanation, we demonstrate that the ranker has a bias toward specific car brands, a bias not evident from local explanations.
\Negin{table ref not working}

% \subsection{Version 2}
% \input{table/cuda_ex}

% As an example, for the query-document pair shown in Table~\ref{tab:qd_cuda}, a feature-based local explanation~\cite{} attributes a significant weight to the term ``Cud'' within the passage.
% This behavior seems highly reasonable for the ranker. However, through our proposed global explanation, we found that the ranker would incorrectly predict ``cuda'' to be relevant to ``cud'', a abnormal behavior not evident from local explanations.

% \subsection{End of Version 2}

% Note that the available MSMARCO corpus or query sets does not contain any of the example that are in the table, thus this behavior would not have been even tested if we had not assessed the relevance thesaurus.

% To the best of our knowledge, there are no global explanations for retrieval models with text inputs such as Transformer-based models.
% Existing global explainers~\cite{} usually are of the form of rules on tabular features ...

% \Negin{I liked the Honda example better as the problem can't be detected from local exp. With this example, if this happens even after deployment, the problem is evident from local exp.}

% The example in \autoref{tab:qd_cuda} shows the abnormal relevance scoring from the state of the art relevance predictor~\footnote{We used a publicly available model from huggingface.co, named ``cross-encoder/ms-marco-MiniLM-L-6-v2''. It was reported to have NDCG@10 of 74.30 on TREC DL 2019.}, where the term matching for the term ``cud'' highlighted. While doc2 seems more more relevant than doc1, as it has exactly the same term, but doc1 actually gets higher score because of the term ``cuda''.

\input{table/ex_table}

Such failure case is hard to discover when this query/document pair is not  included in the evaluation set. 
It is not practical to enumerate all possible queries and annotate all query-document pairs. Even the counter factual explanation methods~\cite{guidotti2022counterfactual, poyiadzi2020face} cannot find this  because they are limited to local examples.  \Negin{this -> this bias?}
Human intervention is required to judge if this is abnormal or not.  \Negin{this -> this bias} \Negin{human also needs to find it from the relevance thesaurus, right?}

This is identified based our global explanation, relevance thesaurus as listed in table~\ref{ex:table}.  \Negin{to go to the end of the paragraph ``a bias not evident from local explanations.''?}

Our goal is to globally explain the behavior of  Transformer-based ranking models. 
For this purpose, we propose to distill their term matching behavior and build a \emph{relevance thesaurus} that specifies the semantic relevance degree between each pair of terms. 
The format of explanation is motivated by the fact that global explanations of information retrieval models primarily need to focus on features from query-document interaction, query-independent, or document-independent features.
More specifically, local explanations that are \emph{specific} to a query can be based on different types of explanation features: tokens, terms, phrasal concepts, or engineered features. However, global explanations generally cannot work by listing important terms or phrases of a document since their importance can change from a query to another.
Term matching is among the most important relevance features of the query-document interaction type. Thus, we build a relevance thesaurus to globally explain the behavior of retrieval models. 

% Limitation of existing methods
Most of existing term-level modeling works have limitation to work as global explanations. 
\Negin{term-level modeling works -> term-level retrieval models? or most of existing works to obtain term relevance relationships?}
Traditional translation models~\cite{} rely on corpus co-occurrence statistics to infer semantically relevant terms. They do not benefit from contextual representations by neural language models or from large training data for relevance ranking. 
Neural translation model~\cite{boytsov2021exploring} and Splade~\cite{} are restricted to  unigrams in BERT's subword vocabulary. They  are not applicable for terms that are composed of multiple subwords. 
Recent retrieval models based on neural language models mostly encode the entire query or document to get vector representations~\cite{khattab2020colbert} or extension terms~\cite{nogueira2019doc2query}, which do not allow us to predict if the identified matched tokens appear in different contexts. \Negin{recent retrieval models may be better to be moved after the second challenge, it seems hard to understand it without that description.}

Moreover, there was little effort to use term-level models as explanations for more complex like cross-encoder architectures.
(It is a snake's leg?) \Negin{what does this mean?}
% boytsov - pronounce as buy-chof

% Having globally faithful explanations is much more challenging  than locally faithful ones. 


First challenge of building a global relevance thesaurus lies in the large size of the vocabulary, coupled with the sparsity of term pairs within relevant query-document pairs.
Second, term pairs that are locally important in predicting relevance of a document to a query may not be globally important. 
[example?] \Negin{remove this or replace with example}
Thus, our goal is to build non-contextual semantically relevant term pairs that can be used in all contexts. 



To address these challenges, we propose \modelname\ that iteratively distill the self-attention and relevance knowledge of full cross-attention ranking model~\cite{} into a sparse neural retrieval model. The distilled sparse neural retriever  is then used to build a relevance thesaurus as the global explanation of the ranker. 
More specifically, ... and then filtering to address the second challenge \Negin{remove or complete this}



In addition to the advantages of global explanations, our explanation based on relevance thesaurus paves the path of developing interpretable first-stage retrieval models addressing the challenge of existing dense retrieval models in the zero-shot setting. This advantage is confirmed by our experiments on the zero-shot performance of semantic matching based on distilled relevance thesaurus as explanations.

\Negin{a last paragraph about experimental results}

 


 






==> Draft/2_related.tex <==
\section{Related works}
We begin by reviewing works on the explainability of information retrieval models as well as existing global explanations for other related tasks. 
Our study is closely related to research addressing the vocabulary mismatch problem~\cite{croft2010search}. We, therefore, review various solutions to this problem, categorizing them into traditional information retrieval methods and information retrieval models based on contextual language models.
Finally, as our global explanations reveal some biases in the ranking models, we review studies on this topic. 



\subsection{Global Model Explanations}

Decision trees are widely used as global explanations of neural networks~\cite{boz2002extracting}. \Negin{more ref when it's common}

\subsection{Traditional Information Retrieval}
% Vocabulary mismatch problem was big problem in traditional information retrieval methods.
One widely used technique for vocabulary mismatch is query expansion, which expands the original query with additional terms.
Query expansion is often based on  term co-occurrences~\cite{jing1994association, xu2000improving}, and pseudo-relevance feedback (PRF) is one of the most popular techniques. 

\citet{berger1999information} adopted an idea of the statistical machine translation model~\cite{brown1990statistical} into the language model framework~\cite{ponte1998language} to handle vocabulary mismatch. 
% A query is viewed as a translation of the document, and relevance probability is estimated based on probability that the query is translated from the given document. 
The  probability of a query term translated into a specific document term is estimated based on the co-occurrence statistics in the collection.
Rather than relying on the statistical co-occurrences of terms, we utilize contextual representations from language models to build context-independent relevant term pairs. 
 
\subsection{Neural Information Retrieval}

Fine-tuning pre-trained language models, such as BERT~\cite{devlin-etal-2019-bert}, has proven to be effective for information retrieval~\cite{macavaney2019cedr}. 

There are two main categories of retrieval methods which are purely based on distributed representations. 
The first category is the cross-encoder architecture~\cite{dai2019deeper}, which takes the concatenation of a query and document as input. This architecture allows  cross-attention between all query and document tokens.
The second category is the bi-encoder architecture~\cite{formal2021splade}, where  queries and documents are  separately encoded into dense vectors. The score of documents are then calculated based on the similarity of their vectors to the query vector. 
These methods do not readily provide which query tokens are matched against which document tokens.

Few studies have proposed a method to explicitly identify the relevance relation between query and document terms in order to construct a relevance scoring or retrieval function. 

First group is neural sparse retrieval models that exploit contextual representation of tokens \Negin{or terms?} for sparse retrieval. \Negin{needs citations}
Second group is neural models for query~\cite{naseri2021ceqe} or document~\cite{nogueira2019doc2query} expansion, which use LLMs to add terms to the bag of word representations of the query or document. The expanded query is then used with lexical matching retrieval models to retrieve documents.  
These methods  do not explain which of the original query term and which original document terms are related, because retrieval and scoring is done by expanded query (document) terms. \Negin{I don't get the point of mentioning this group as few studies that match, and say it still does not}
 Moreover, these expansions are only applicable for individual query and document, cannot be used to describe global matching behavior for the retrieval system. 

 Multi-vector retrieval models, such as ColBERT~\cite{khattab2020colbert} and COIL~\cite{gao2021coil}, are a special case of bi-encoder. These models construct vector representations for each token in both the query and the document. 
 The similarity between the vectors of the query and  document tokens is used to score the document.
 While these models offer token-level similarity scores, it is important to note that these scores do not directly correlate with the semantic similarity of their respective tokens.
 This is because token representations are constructed considering the context provided by other tokens. 
 % Thus, the same token may have different representations across various documents, and we cannot acquire relevant terms from these models.

Splade~\cite{formal2021splade} is a sparse retrieval method, which encodes queries and documents into sparse vectors.
Each vector's dimension is aligned with a subword vocabulary of BERT. 
However, this encoding process still exhibits unpredictability; the impact of specific tokens on the encoded vector's dimensions is not straightforward.
For example, the inclusion of the token ``is'' in the input does not guarantee a high weight for ``is'' in the corresponding dimension of the output vector.

All of methods described above incur additional computational and/or storage overhead compared to the traditional retrieval. Bi-encoder models including Splade, require encoding all the corpus with the expensive neural network and storing the vector representations.
Also, the storage required for the encoded vectors can be much larger than the storage for original documents. Efficient neural encoding of query or document requires special hardware acceleration, which is not be available in traditional servers. 

In contrast, the output model of our work is a relevance thesaurus that indicates relation between the terms that are compatible to the traditional indexing architectures, and thus can be seamlessly augmented into existing infrastructures. Moreover all the computational overheads are during the training phase and does not incur significant overheads during the indexing or inference time.


\citet{boytsov2021exploring} extended the idea of translation language model\cite{berger1999information} by using BERT~\cite{devlin-etal-2019-bert} to estimate translation probability. The translation probability is estimated using a multilayer perceptron (MLP) model, where input is the concatenation of the (sub)word embeddings of the query term and document term. The MLP is trained end-to-end using the pairwise loss on MSMARCO training dataset. To make the model robust, this subword-level translation language model was combined with word-level (space-tokenized) BM25 scores to make it more robust. This work does not provide solution for how to model translation probability for the terms that are composed of multiple subwords in BERT's tokenization. Moreover, this model only uses the word-embeddings components of BERT and does not exploit full capacity of the Transformer network.


\subsection{Biases or ranking model}


The Transformer-based text modeling methods are 


 



==> Draft/3_method.tex <==
\section{Method}
\label{sec:rel_term_metric}



% The goal is to distill term pairs in a given query and document that are matched by a retrieval model using a contextualized language model. [from a full cross-encoder~\cite{}.]

Our goal is to globally explain the term matching behavior of the full cross-attention ranking model~\cite{} that takes the concatenation of a query and document as input and models their interaction for building their representations. 

The first solution to obtain matched terms between a query and document is to use self-attention weights. However,  there are contradictory findings about using attention values as explanations~\cite{}. 
\Negin{specific reason why they can be not optimal for semantic matching?}


Another solution is using token-level dual encoder models, such as ColBERT~\cite{}. However, it has beens shown that  that dot product similarity of token representations from dual encoders are not effective for modeling term-level relevance~\cite{boytsov2021exploring}.

% There are two main architectures utilizing contextualized language models for relevance prediction: (1)~
% dual encoders~\cite{} that represent a query and document independently, and 
% (2)~full cross-attention~\cite{} that takes the concatenation of a query and document as input and models their interaction for building their representations. 

 




To address these challenges, we propose  relevance prediction based on a new interaction scheme between a query and document. Our proposed model is based on cross-attention between segments of a query and document, which we refer to as \emph{Partial Cross-Encoder}~(\modelname). 
Partial cross-attention allows to localize the impact of self-attention in Transformer [not impacting other tokens]


We train \modelname\ in two steps to distill a global table of semantic term relevance from the full cross-encoder. 






\subsection{ Training Initial PaCE Model}
In the first distillation step, 
PaCE is used to score a query-document pair by generating scores for two inputs from a given query and document.
Each input consists of concatenating a segment from both the query and the document, and is then scored through cross-attention. 
These two scores are summed as the relevance score for the query-document pair.



More specifically, query $q$/$d$ is partitioned into non-overlapping segments $q_1$/$d_1$ and $q_2$/$d_2$, the combination of which reconstructs the original query $q$/$d$.

In the first distillation step, the score for a given query and document is calculated as
% \begin{equation}
% S(q,d) = \sum_{i \in \{1,2\}}
%      W \cdot \mathrm{PaCE}_{\mathrm{[CLS]}}(q_i [\mathrm{SEP}] d_i) + b
% \end{equation}
\begin{equation}
PaCE(q_i,d_i) = 
     W \cdot \mathrm{BERT}_{\mathrm{[CLS]}}(q_i [\mathrm{SEP}] d_i) + b, 
     \label{first-pace-scoring-eq}
\end{equation}
\begin{equation}
S(q,d) = S(q_1, d_1) + S(q_2, d_2)
\end{equation}
In this scoring scheme following the full cross-attention ranker~\cite{bert}, a linear layer is added on top of the [CLS] representation obtained for the concatenated $q_i$ and $d_i$. 
As a result, two  relevance scores are predicted  for each pair ($q_1$, $d_1$) and ($q_2$, $d_2$).
The scores obtained for partial segments are then summed to predict the overall relevance score of $q$ and $d$.






\Negin{we can call this the first student model}


\textbf{Distilling Self-Attention of Full Cross-Encoder.}
Based on the query segments, document $d$ is partitioned such that $d_1$/$d_2$ most likely contains the document part relevant to $q_1$/$q_2$. 
To estimate which tokens of $d$ are relevant to $q_1$, we use the attention scores from the full cross-encoder ranker~\cite{}, which takes the concatenation of the entire $q$ and $d$ as its input. 
$d_1$ is built by selecting document tokens that have high attention scores to tokens of  $q_1$.
We randomly sample how many tokens are to be selected, which can range from one to all tokens of $d$. \Negin{if the top scoring tokens are not continuous then what is the selection criteria?} [It avoids splitting subwords, by taking max score of them as representative score. In other case, it may not be continuous]
Partial segments include the cases where the segment of the query and document contains only a single term. 






\textbf{Training of PaCE.}
PaCE is initialized with pre-trained BERT, similar to the full cross-attention ranking model~\cite{}.
% using query-document relevance labels based on predicting a relevance score for a pair of partial query and partial document. 
% $R_{PaRM}$ is 
% trained 
Given a query $q_i$, a relevant document $d_i^+$, and non-relevant document $d_i^-$, PaCE is trained using pairwise hing loss function as 
\begin{equation}
\mathcal{L} = \max\left(0, 1 - S(q_i, d_i^+) + S(q, d_i^-)\right),
\label{hinge-loss-fn-eq}
\end{equation}
where $s(q,d^*)$ is calculated using Eq.~\ref{}.

 

\textbf{Global Table from Initially Trained PaCE.}

Once \modelname\ is trained, it can be to score a short query or document span, including single terms. 


For a pair of query and document, where a query term $qt$ does not have exact match in the document, all document terms are scored against $qt$ using Eq.~\ref{first-pace-scoring-eq}, $S(qt, dt)$.
The document term $dt$ with the highest score is paired with $qt$. 
The obtained pairs are referred to as \Negin{a notation like $\mathcal{M}$, contains X pairs}

The initial global relevance thesaurus $\mathcal{M}$ is used as training data for the second training stage of \modelname.



[Training PaRM is a prerequisite for TeRM for several reasons. First, it is unclear which query and document terms are relevant, and attempting to supervise all term-pair combinations within a query and document could result in noisy supervision. Second, training on term-level relevance is more prone to overfitting than with longer, but pre-training with larger contexts (PaRM) improves overall performance .]

\subsection{Fine Tuning PaCE Model for Explicit Term Matching}


The first student model learns to assign a higher score to more relevant segment pairs. 
The scores  for term pairs in $\mathcal{M}$ are not calibrated to a specific range. This makes it challenging to select a threshold value for filtering out term pairs that  are not relevant in  all contexts. 


In the second stage, PaCE is used as a sparse retrieval model by predicting the semantic relevance between a query and document term on a scale of 0 to 1. 
\begin{equation}
    PaCE(qt, dt) = Sigmoid(W \cdot BERT_{\mathrm{CLS}}(qt \mathrm{[SEP]} dt) + b)~\label{term_sidmoid}
\end{equation}
The sigmoid layer on top of the  [CLS] representation ensures the scale of the score. 

\begin{equation}
    S(q,d) = \sum_{qt \in d}{ \mathrm{TF}(qt) \cdot \mathrm{IDF}(qt)} + \sum_{qt \notin d} R(qt, dt) \cdot \mathrm{TF(dt)} 
    \label{eq:BM25T}
\end{equation}



\textbf{Training of PaCE.}
Pre-trained PaCE from the first stage is fine-tuned using the hinge loss function provied in Eq.~\ref{hinge-loss-fn-eq}.





\Negin{a separate section on the modified BM25?, the PSQ method can help \url{https://dl.acm.org/doi/pdf/10.1145/860435.860497}}

==> Draft/pre_intro.tex <==
\section{Introduction}

\subsection{Motivation}

To improve the interpretability of deep neural network based information retrieval (IR) models, 

\Negin{why global explanation of IR models}

\Negin{an example that local explanation of matching car in the query with car brand in doc seem reasonable, but does not reveal the bias as the global explanation does. }

\Negin{why term alignment explanation for interpretability and not other formats of explanations?}



\subsection{Problem}

The outcome of this process is a term-pair table along with a scoring function. Together, they constitute a shallow model. This model serves two purposes: functioning as model explanations and operating as an independent scoring function.

\textbf{Model explanation }
The criteria of relevance can be replaced with other criteria such as a blackbox ranking model's ranking predictions as a standard of relevance, so that the identified term pairs can work as an global explanation for the particular model.
The term pairs provide lexical explanation that give insights about the model behavior, which can be used to find out existence of the bias or weakness of the model. Ideally, the BM25 scoring function, which works as a criterion for term pairs can be replaced with more complex functions to better approximate the blackbox model's behavior.

\textbf{Independent scoring function }
The identified term pairs can also be employed as an independent scoring function. First, this function would be useful as a lightweight search function, such as as initial phase of retrieval, or in systems which have strict restriction of storage or computations. Second, in systems where manual intervention in search criteria is desirable, non ML-expert can easily modify the table to change the behavior of the search system.


\subsection{Previous Work don't solve it (optimally)}


\subsection{Challenges}

While some query term and document pairs are very strong indicators of relevance that are likely to be referring to the same concept, some term pairs are only indicative of relevance when certain contexts exist to disambiguate meaning. Thus, the term alignments that are provided to the users or to system administrators, need to be either filtered with specific criteria, or accompanied with additional information that indicates what that alignment implies.

First, it is challenging to directly search for relevant term pairs due to the sparse occurrence of the query-term and document-term pairs in relevant documents. Thus, we use distributed representations as intermediate data structures to search for the relevant term pairs.

Given a relevant query-document, it is not easy to predict which term pairs are promising relevant pairs. Treating all term pairs as potential candidates and applying uniform gradient updates or occurrence counting tends to introduce noise into the supervision. This approach could necessitate an impractical amount of training data or lead to overfitting.


\subsection{Summary of Proposed Model}
In this work, we introduce \peptt , a novel approach for identifying relevant query-term and document-term pairs in the passage ranking tasks. Our approach trains a term-pair relevance predictor by fine-tuning BERT, which is then used to build a term-pair table. 

The term-pair relevance predictor is trained with two phases.
In the first phase, we train a PAT model which was proposed in previous chapter. This model scores a query-document pair by generating scores from two partial observations, each consisting of subsets of the query and document. The final relevance score for the query-document pair is the sum of these two scores.
The PAT model is trained using query-document relevance labels. It is capable of predicting relevance score to a given partial query and partial document pair, including the case that each of the partial query and document is a single term. The PAT model is trained to assign higher scores to more relevant pair, but its output scores are not calibrated to be used in the BM25 scoring function. In the second phase, we fine-tune PAT model as a regression model which scores a given query and document term pair with an objective of optimizing BM25 augmented effectiveness. The trained regression model is used to score possible term pairs to build a term-pair table with the scores for each pair.




\subsection{Advantages of the Proposed Model}


\subsection{Evaluation}

In the machine learning context, it was argued that if a shallow model, such as decision tree, can predicts the outputs of a complex deep neural network models, the shallow model work as global explanation that explain the deep models behavior~\cite{craven1995extracting, guidotti2018survey}.

The fidelity of a relevance thesaurus in explaining the target ranker can be evaluated by augmenting it into a traditional IR system, which relies on the frequency of query terms in documents. Traditional IR systems are known to suffer from a vocabulary mismatch problem. Augmenting relevance thesaurus into a traditional IR model will improve their effectiveness and ideally result in a higher correlation with the complex Transformer-based rankers. 



 As a benchmark for measuring the effectiveness, we use a traditional term-matching based scoring function, BM25, and use the found relevant terms as the same term of the scoring function. While BM25 may not be the optimal scoring function to explain relevance mechanism, it serves as initial criteria in our study to determine the relevance of the term pairs. 

\Negin{Correlation between BM25 and BERT rankings as evaluation?}

\subsection{Summary of the Results}
Our experiments using the MSMARCO training dataset led to the discovery of 150,000 term pairs. Incorporating these pairs into the BM25 model resulted in a significant improvement in the Mean Reciprocal Rank (MRR) score. Specifically, there was an increase of 2.3\%, a notable improvement compared to the 1.0\% increase achieved solely through stemming.

Further analysis of the term pairs revealed potential biases in passage ranking models. Specifically, biases were observed in 
how different automotive brand names were associated with a generic category term. For instance, in the automotive sector, we show that the table has a large magnitude of gap between the scores for the generic query term ``car'' and different car brand names. Our analysis showed that these brand name biases are also consistently observable in the complex, state-of-the-art ranking models, demonstrating the potential of the shallow models in discovering potential biases.

==> abstract.tex <==

\begin{abstract}
To improve the interpretability of deep neural network based information retrieval (IR) models, we explore the direction of explaining these models by building a relevance thesaurus . 
The relevance thesaurus expresses which document terms will be a strong indicator of relevance with respect to a specific query term or phrase. 
The fidelity of a relevance thesaurus as an explanation is evaluated by measuring the correlation gain when it is augmented into a traditional IR system to address vocabulary mismatch. 
To build the relevance thesaurus, we propose a novel method of training a Transformer model which takes only parts of a query and document as input to predict relevance. Our experiments demonstrate that the proposed model reliably predicts the degree of relevance between the query and document terms. Moreover, further analysis reveals biases in passage ranking models, particularly in how automotive brands are associated with the generic term ``car'', indicating that even the state-of-the-art models show consistent brand name biases, demonstrating the effectiveness of our method in identifying such biases.

\end{abstract}

==> figures/append_test2.tex <==

\begin{tikzpicture}
\begin{axis}[
    ybar,
    bar width=2mm,
    width=0.5\textwidth,
    height=8cm,
    xlabel={Added letters},
    ylabel={Score changes},
    ymin=-0.1, ymax=0.2,
    xtick=data,
    xticklabels={a, b, c, d, e, f, g, h, i, j, k, l, m, n, o, p, q, r, s, t, u, v, w, x, y, z},
    x tick label style={rotate=0, anchor=north},
    ymajorgrids=true,
    grid style=dashed,
]
\addplot[draw=black, fill=blue!10] coordinates {
    (0,-0.00820500080932876) (1,0.1310710813887343) (2,0.12529361468113348) (3,0.1347097317258755) 
    (4,0.1130408585190535) (5,0.12341313587572285) (6,0.11546545212497254) (7,0.16372339276340372) 
    (8,0.1285384099878475) (9,0.1429567006593217) (10,0.15901448331520468) (11,0.15293433078510796) 
    (12,0.08745833568111389) (13,0.12658730580540237) (14,0.11090059040073387) (15,0.17859506108770204) 
    (16,0.14398081966502937) (17,0.1471543980617366) (18,0.05467552363039729) (19,0.1542828060433774) 
    (20,0.0991452518337501) (21,0.134283896740117) (22,0.12002501041886811) (23,0.15576012090532604) 
    (24,0.15928329867933563) (25,0.12278295811005457)
};
\end{axis}
\end{tikzpicture}

==> figures/parm_train_old.tex <==

\begin{figure}[htb]
    \centering
    \begin{tikzpicture}[node distance=0mm]
        \tikzset{Token/.style={rectangle,minimum height=6mm, minimum width=8mm,}}
        \tikzset{QToken/.style={Token, fill=red!10, font=\small}}
        \tikzset{DToken/.style={Token, fill=blue!10, font=\small, minimum width=15mm}}
        \tikzset{QLine/.style={->, thick, red!40}}
        \tikzset{DLine/.style={->, thick, blue!40}}
        \tikzset{Predictor/.style={rectangle,draw,minimum width=2.5cm,minimum height=1cm}}    
        \tikzset{Prediction/.style={rectangle, fill=black!10, minimum height=3mm, minimum 
        width=3mm, font=\small}}
            
        \matrix[anchor=west, row sep=1mm] (left_tower) {
            \node[Prediction] (z1){$\rho_1$}; \\ [1mm]
            \node[Predictor] (ls1) {PaRM}; \\
            \node(q1)[QToken]  {$q_1$}; 
            \\
        };
        \node(d1)[DToken, minimum width=10mm, fill=blue!10, right=of q1] {$d_1$}; 
        
        \node[above=15mm of d1] (zs) {};
        \draw[<-] (z1.south) -| ++(0, -0.20);
    
        \node[right=of left_tower] (center) {};
        \matrix[anchor=west, row sep=1mm, right=of center] {
            \node[Prediction] (z2){$\rho_2$}; \\ [1mm]
            \node[Predictor] (ls2) {PaRM}; \\
            \node(q2)[QToken]  {$q_2$}; 
            \\
        };
        \node(d2)[DToken, minimum width=7mm, fill=blue!10, right=of q2] {$d_2$}; 
    
        \node[QToken, below=1em of left_tower] (qtext1) {who is [MASK]};   
        \node[QToken, below=0.5mm of qtext1] (qtext2) {[MASK] Plato};
        % \node[QToken, below=1em of qtext2] (qtext) {who is Plato};   
    
        \node[DToken, right=2em of qtext1] (dtext1) {[MASK] was a Greek philosopher.};
        \node[DToken, right=2em of qtext2] (dtext2) {Plato was a Greek [MASK] .};
        % \node[DToken, right=2em of qtext] (dtext) {Plato was a Greek philosopher.};
        
        % \draw[->] (qtext1.west) -- ++(-0.5, 0) -- ++(0, 0.6)  |- (q1.west);
        \draw[QLine] (qtext1.north) -- ++(left:1em) -| (q1);
        \draw[QLine] (qtext2.east) -- ++(right:1.5em) -- ++(up:3em) -|  (q2);
        
        % \draw[QLine] (qtext.west) -- ++(-0.4, 0.0) -- ++(0, 0.8)  |- (qtext1.west);
        % \draw[QLine] (qtext.west) -- ++(-0.4, 0.0) -- ++(0, 0.8)  |- (qtext2.west);
        
        
        \draw[DLine] (dtext1.west) -- ++(left:1.5em) -- ++(up:1.5em) -| (d1);
        \draw[DLine] (dtext2.east) -- ++(right:3em) -- ++(up:3em) -| (d2);
    
        % \draw[DLine] (dtext.west) -- ++(-0.2, 0.0) -- ++(0, 0.8)  |- (dtext1.west);
        % \draw[DLine] (dtext.west) -- ++(-0.2, 0.0) -- ++(0, 0.8)  |- (dtext2.west);
    
        
        \node[rectangle,draw, right=7mm of z1] (combine) {\small{$Sum$}};
        \node[Prediction, above=2mm of combine] (y) {$y$};
        \draw[<-] (z2.south) -| ++(0, -0.20);
    
        \draw[->] (z1) -- (combine);
        \draw[->] (z2) -- (combine);
        \draw[->] (combine) -- (y);
     
    \end{tikzpicture}
      \caption{The first stage training of PaRM. The query ``who is Plato'' (red) is partitioned into $q_1$ and $q_2$. The document ``Plato was a Greek philosopher'' (blue) is masked to generate $d_1$ and $d_2$.}
    \label{fig:parm_train}


    \begin{tikzpicture}[node distance=0mm]
        \tikzset{Token/.style={rectangle,minimum height=6mm, minimum width=8mm,}}
        \tikzset{QToken/.style={Token, fill=red!10, font=\small}}
        \tikzset{DToken/.style={Token, fill=blue!10, font=\small, minimum width=15mm}}
        \tikzset{Predictor/.style={rectangle,draw,minimum width=2.5cm,minimum height=1cm}}
        \tikzset{Prediction/.style={rectangle, fill=black!10, minimum height=3mm, minimum width=3mm, font=\small}}    
        \matrix[anchor=west, row sep=1mm] (left_tower) {
            \node[Prediction] (z1){$\rho$}; \\ [1mm]
            \node[Predictor] (ls1) {PaRM}; \\
            \node(q1)[QToken]  {who}; 
            \\
        };
        \node(d1)[DToken, minimum width=10mm, fill=blue!10, right=of q1] {philosopher}; 
        \node[above=15mm of d1] (zs) {};
        \draw[<-] (z1.south) -| ++(0, -0.20); 
    \end{tikzpicture}
    \caption{The final PaRM model predicts a relevance score for a query term ``who'' and document term ``philosopher'', which is used to build a relevance thesaurus.}
    \label{fig:parm_term}
\end{figure}

\begin{figure*}
    
\end{figure*}


==> figures/pat_ir_model.tex <==

\begin{figure}[htb]
    \centering
    \begin{tikzpicture}[node distance=0mm]
    \tikzset{Token/.style={rectangle, fill=blue!10,minimum height=4mm, font=\small}}
    \tikzset{QToken/.style={rectangle, fill=red!10,minimum height=4mm, minimum width=12    mm, font=\small}}
    \tikzset{PToken/.style={rectangle, fill=blue!10,minimum height=4mm, minimum width=12    mm, font=\small}}
    \tikzset{Predictor/.style={rectangle,draw,minimum width=2.5cm,minimum height=1cm}}
    \tikzset{Prediction/.style={rectangle, fill=black!10, minimum height=3mm, minimum 
    width=3mm, font=\small}}
        
    \matrix[anchor=west, row sep=1mm] (left_tower) {
        \node[Prediction] (z1){$\rho_1$}; \\ [1mm]
        \node[Predictor] (ls1) {BERT}; \\
        \node(q1)[QToken]  {$q_1$}; 
        \\
    };
    \node(d1)[Token, minimum width=10mm, fill=blue!10, right=of q1] {$d_1$}; 
    
    \node[above=15mm of d1] (zs) {};
    \draw[<-] (z1.south) -| ++(0, -0.20);

    \node[right=of left_tower] (center) {};
    \matrix[anchor=west, row sep=1mm, right=of center] {
        \node[Prediction] (z2){$\rho_2$}; \\ [1mm]
        \node[Predictor] (ls2) {BERT}; \\
        \node(q2)[QToken]  {$q_2$}; 
        \\
    };
    \node(d2)[Token, minimum width=7mm, fill=blue!10, right=of q2] {$d_2$}; 

    \node[font=\footnotesize, rectangle, fill=red!10, below=of left_tower] (qtext1) {who is [MASK]};   
    \node[font=\footnotesize, rectangle, fill=red!10, below=0.5mm of qtext1] (qtext2) {[MASK] Plato};
    
    \node[font=\footnotesize, rectangle, fill=blue!10, minimum height=4mm, right=of qtext1] (dtext1) {[MASK] was a Greek philosopher.};
    \node[font=\footnotesize, rectangle, fill=blue!10, minimum height=4mm, right=of qtext2] (dtext2) {Plato was a Greek [MASK] .};
    
    \draw[->] (qtext1.west) -- ++(-0.5, 0) -- ++(0, 0.6)  |- (q1.west);
    % \draw[->] (qtext2.east) -- ++(+1.0, 0) -- ++(0, 0.9)   -| (q2);
    
    \draw[->] (dtext1.north)  ++(-2, 0) -- ++(0, 0.3)  |- (d1);
    \draw[->] (dtext2.east) -- ++(1.2, 0.0)  |- (d2.east);
    
    \node[rectangle,draw, right=7mm of z1] (combine) {\small{$Sum$}};
    \node[Prediction, above=2mm of combine] (y) {$y$};
    \draw[<-] (z2.south) -| ++(0, -0.20);

    \draw[->] (z1) -- (combine);
    \draw[->] (z2) -- (combine);
    \draw[->] (combine) -- (y);
 
    \end{tikzpicture}
      \caption{The architecture of proposed \modelname\ model for the first stage training.
      % $q_1$ and $q_2$ are two subsets of query tokens. $d_1$ and $d_2$ are the subsets of document tokens.
      }
    \label{fig:local_decision2}

\end{figure}



==> figures/when_year_png.tex <==

\begin{figure*}
    \centering    
    \includegraphics[width=0.9\textwidth]{figures/When_2015.png}
    \caption{The left axis shows the scores in our relevance thesaurus for the query term ``when'', and the document term as years from 2000 to 2024. The right axis shows the scores from the cross encoder model for query-document pairs with ``when'' and year mentions.}
    \label{fig:when_2015}
\end{figure*}

==> old_1_1_intro.tex <==

\section{Introduction}


% Backgrounds about ranking models and specific example for motivation
Relevance models are built by fine-tuning LLMs with relevance supervisions like as MSMARCO. These models are effective in handling semantic matches between query and document, which describes the query term does not exist in the document, but have other semantically related term or expression in it. However, it is hard to grasp the degree of semantic match and limitations of these semantic matching behavior. For example, we can expect that the BERT cross-encoder model can match the query term ``car'' to similar terms like ``vehicles'' or even to a specific brand name like ``ford'', but will not match it to irrelevant looking term ``\underline{car}a''. 
However, there is no systematic way to find out such information, or verify such behaviors.

\input{table/ex_table}

% Model explanation background (ML)
This challenge of model explanation, has been studied in machine learning perspectives. Explaining model behaviors is considered as seeking for a shallow and interpretable model representations, such as decision trees, which predicts the outputs of a targeted blackbox models to be explained~\cite{craven1995extracting, guidotti2018survey}. For a classification task on tabular features, explanation can be interpreted as rules like having certain values combinations for certain feature set will result in positive predictions. 

% Connect model explanation with our specific goal
If we apply this paradigm to IR tasks, explanation could be like having certain terms in query and having certain terms in document will results in relevant predictions. This is very similar to building relevance thesaurus in traditional IR works (cite). If such explanation is available, they can be used to improve the traditional IR models. 

% State concrete goal
We explore the direction of explaining these models by building a relevance thesaurus . 
We assume that we are given relevance signals, which can be expressed as a list of (query, document, score) triplets. The relevance signals could be either from relevance training data such as MSMARCO, or from other neural ranking models such as cross-encoder style rerankers. 
Our goal is to come up with a relevance thesaurus, which is composed of a list of (query term, document term, score) triplets, where the score indicate how strongly this term pair indicates relevance. 

% Evaluating quality
The fidelity of a relevance thesaurus in explaining the target ranker can be evaluated by augmenting it into a traditional IR system, which relies on the frequency of query terms in documents. Traditional IR systems are known to suffer from a vocabulary mismatch problem. Augmenting relevance thesaurus into a traditional IR model will improve their effectiveness and ideally result in a higher correlation with the complex Transformer-based rankers.  

% Duplicate
 As a benchmark for measuring the effectiveness, we use a traditional term-matching based scoring function, BM25, and use the found relevant terms as the same term of the scoring function. While BM25 may not be the optimal scoring function to explain relevance mechanism, it serves as initial criteria in our study to determine the relevance of the term pairs. 

The acquired relevance thesaurus can be used by developers, system administrators or related authorities. To examine possible biases need to be either filtered with specific criteria, or accompanied with additional information that indicates what that alignment implies.

% Value of this work

The outcome of this process is a term-pair table along with a scoring function. Together, they constitute a shallow model. This model serves two purposes: functioning as model explanations and operating as an independent scoring function.

\textbf{Model explanation }
The criteria of relevance can be replaced with other criteria such as a blackbox ranking model's ranking predictions as a standard of relevance, so that the identified term pairs can work as an global explanation for the particular model.
The term pairs provide lexical explanation that give insights about the model behavior, which can be used to find out existence of the bias or weakness of the model. Ideally, the BM25 scoring function, which works as a criterion for term pairs can be replaced with more complex functions to better approximate the blackbox model's behavior.

\textbf{Independent scoring function }
The identified term pairs can also be employed as an independent scoring function. First, this function would be useful as a lightweight search function, such as as initial phase of retrieval, or in systems which have strict restriction of storage or computations. Second, in systems where manual intervention in search criteria is desirable, non ML-expert can easily modify the table to change the behavior of the search system.

% Technical challenge and solutions
There are two challenges in identifying relevant term pairs.
% Problem 1 - Sparsity - we use neural model for fine-tuning
First, the vocabulary size and sparsity of query-document term pair combinations occurrence makes hard to have sufficient observations for each term-pair. For example, MSMARCO contains a few million unique terms, which could make trillion term pair combinations while there are only half million relevant query-document pair. 
This can be solved by incorporating neural models. 

% problem 1 - Sparsity
It is challenging to directly search for relevant term pairs due to the sparse occurrence of the query-term and document-term pairs in relevant documents. Thus, we use distributed representations as intermediate data structures to search for the relevant term pairs. We train a neural model, which can predict relevance score for the given query and document term pairs. 

Given a relevant query-document, it is not which term pairs are relevant pairs. Treating all term pairs as potential candidates and applying uniform gradient updates or occurrence counting tends to introduce noise into the supervision. This approach could necessitate an impractical amount of training data or lead to overfitting.
We solve this problem by gradually decreasing the input scope of the relevance model, from entire query-document pair to partial spans of query/document and individual query term and document term pairs. 

The resulting relevance model predicts the relevance scores for the given term pairs, and we acquire relevance thesaurus by scoring possible term-pair combinations.

Further analysis of the term pairs revealed potential biases in passage ranking models. Specifically, biases were observed in 
how different automotive brand names were associated with a generic category term. For instance, in the automotive sector, we show that the table has a large magnitude of gap between the scores for the generic query term ``car'' and different car brand names. Our analysis showed that these brand name biases are also consistently observable in the complex, state-of-the-art ranking models, demonstrating the potential of the shallow models in discovering potential biases.

The contributions of this work are as follows:
 \begin{enumerate}
    \item We propose that a shallow model can be used as a global explanation for a more complex deep model, when they are trained with similar supervision signal.
    \item We propose an partial segment level relevance modeling architecture which can be used to identify a relevant query-term and document-term pairs from the query-document level relevance signals (\autoref{sec:rel_term_metric}). 
    \item We demonstrate findings from the resulting relevance thesaurus, which includes potential biases of a targeted complex model.
\end{enumerate}


% Move to related work
\subsection{Why previous works doesn't solve it}
Model explanations can be divided into two types: local explanations and global explanations. A local explanation is specific to individual instances, meaning that the importance of features is determined within a particular context and may not be applicable to other situations. Since local explanations are based on context-specific implications, attempting to aggregate them on a global scale (for example, by averaging instances across a dataset) using arbitrary criteria may fail to maintain the underlying principles or goals of the local contexts.

On the other hand, existing global explanations typically apply to single text classification tasks and demonstrate the relationship between certain input features (like words) and output labels. In fields outside of Natural Language Processing (NLP), global explanations often focus on tabular data, highlighting the connection between features and labels. However, these methods are not suitable for explaining relevance models, as importance of the document features (tokens) are highly dependent on the query tokens. 




==> table/corr_score_rank.tex <==
\begin{table}[]
\begin{tabular}{lcc}
\toprule
Model               & Score & Rank  \\ \hline
Cross Encoder       & 0.28  & -0.28 \\
Splade v2           & 0.41  & -0.41 \\
TAS-B               & 0.37  & -0.36 \\
Contriever          & 0.42  & -0.44 \\
Contriever MS MARCO & 0.20  & -0.23 \\
\bottomrule
\end{tabular}
\end{table}

==> table/cuda_ex.tex <==


\begin{table}[h]
    \centering
    \begin{tabular}{c|l}
        \toprule
        Query &  What is \underline{cud} \\ \hline
        Doc 1 & \underline{CUDA} is a parallel computing platform (...) that \\
        (3.6) &  makes using a GPU for general purpose computing simple.  \\ \hline 
        Doc 2 & This process, called “chewing the \underline{cud},” helps sort the \\ 
        (3.0) & digesta and absorb nutrients. \\  \bottomrule
    \end{tabular}
    \caption{Scores for two documents towards the given query. Doc 2 should be considered more relevant, as it describes the actual keyword ``cud''. However, the relevance model (cross encoder) }
    \label{tab:qd_cuda}
\end{table}


==> table/honda_ex.tex <==

\begin{table}[h]
    \centering
    \begin{tabular}{l|l}
        \toprule
        Query &  What is an actuator in a \textbf{car} \\ \hline
        Doc & About \textbf{Honda} door lock actuator, door lock actuator \\ 
        & is the latching mechanism installed in your every single \\
        & door in your ... \\
        \bottomrule 
    \end{tabular}
    \caption{Example query/document}
    \label{tab:qd_honda_actuator}
\end{table}


